E4S: Fine-grained Face Swapping via Editing With Regional GAN Inversion

This paper proposes a novel approach to face swapping from the perspective of fine-grained facial editing, dubbed "editing for swapping" (E4S). The traditional face swapping methods rely on global feature extraction and fail to preserve the detailed source identity. In contrast, we propose a Regional GAN Inversion (RGI) method, which allows the explicit disentanglement of shape and texture. Specifically, our E4S performs face swapping in the latent space of a pretrained StyleGAN, where a multi-scale mask-guided encoder is applied to project the texture of each facial component into regional style codes and a mask-guided injection module manipulating feature maps with the style codes. Based on this disentanglement, face swapping can be simplified as style and mask swapping. Besides, due to the large lighting condition gap, transferring the source skin into the target image may lead to disharmony lighting. We propose a re-coloring network to make the swapped face maintain the target lighting condition while preserving the source skin. Further, to deal with the potential mismatch areas during mask exchange, we design a face inpainting module to refine the face shape. The extensive comparisons with state-of-the-art methods demonstrate that our E4S outperforms existing methods in preserving texture, shape, and lighting. Our implementation is available at https://github.com/e4s2024/E4S2024.

==> fig_tex/StyleGANBasedSwappingComp.tex <==
\begin{figure}[t]
\centering
\setkeys{Gin}{width=1\linewidth}
\captionsetup{belowskip=-10pt}
\begin{subfigure}{1\linewidth}
\includegraphics[width=1\textwidth]{figs/fig_stylegan-cropped.pdf}
\end{subfigure}
\caption{Comparisons with StyleGAN-based face swapping methods.}
    \label{fig:StyleGANBasedSwappingComp}
\end{figure}

==> fig_tex/blending.tex <==
\begin{figure}
  \centering  \includegraphics[width=\linewidth]{figs/blending.jpeg}
  \caption{The illustration of multi-band blending between the swapped face $\hat{I}$ and target $T$.}
  \label{fig:blending}
\end{figure}

==> fig_tex/fig_gradio.tex <==
\begin{figure*}[t]
  \centering
\includegraphics[width=0.95\linewidth]{figs/fig_gradio-cropped.pdf}
  \caption{Illustration of our re-coloring network $B_{\psi}$. In training stage, we use two image augmentation to get the re-colored $I'_{\rm{AG}}$ and flipped $I'_{\rm{A}}$. Their FPN~\cite{zhang2020cross} features $f_{\rm{AG}}$ and $f_{\rm{A}}$ in }
  \label{fig:gradio}
\end{figure*}

==> fig_tex/teaser.tex <==
    \begin{figure*}
      \centering
    \includegraphics[width=0.96\linewidth]{IEEEtran/figs/fig_teaser-cropped.pdf}
       \vspace{-0.2cm}
       \caption{Compared with the existing StyleGAN-based face swapping approaches MegaFS~\cite{zhu2021MegaFS}, StyleFusion~\cite{kafri2021stylefusion}, and HiRes~\cite{xu2022high}, our E4S can achieve high-fidelity swappped results. Note that ours achieves best identity preservation and proper occlusion handling, where the target skin tone is kept and the target lighting condition is well transferred to the swapped results. All the facial images are at $1024\times1024$.} 
       \label{fig:teaser}
       \vspace{-0.2cm}
    \end{figure*}

% TODO: styleface?

==> tex/acknowledge.tex <==
\section*{Acknowledgment}



The authors would like to thank...


==> tex/author_biography.tex <==
\section{Biography Section}
%\vspace{-2cm} 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_lmm.pdf}}]{Maomao Li}
is a PhD student in the computer science from The University of HongKong, directed by Prof. Dong Xu.
Before that, she is a Junior Researcher at Tencent AI Lab, Shenzhen, China, working on face swapping.
She received her master degree in Computer Science from Tsinghua University in 2020.
She got her B.E. degree in communication engineering from JiLin University in 2017. Her main research interests include face swapping, video generation.
\vspace{-1cm}
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_yuange.jpg}}]{Ge Yuan} is now a PhD student in The University of HongKong (TUHK) supervised by Prof. Dong Xu. He received his M.S degree in computer science from Sun Yat-sen University (SYSU) in 2023 advised by Huicheng Zheng and B.S degree in Computer Science from Huazhong University of Science and Technology (HUST) in 2014. 
From Apr. 2022 to Jun. 2023, he worked as a research intern in Tencent AI Lab.
His main research includes diffusion models, face swapping, and face recognition.
\vspace{-1cm} 
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_wcr.png}}]{Cairong Wang} graduated from Shenzhen International Graduate School of Tsinghua University in 2023 with a Master's degree in Computer Technology. He received his bachelor's degree in Computer Science and Technology from Beijing Institute of Technology. He is currently working as an algorithm engineer in BYD Basic Science Research Institute. His main research work is on  face swapping and image inpainting.
\vspace{-1cm} 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_lza.jpg}}]{Zhian Liu} received his master degree in computer science from South China University of Technology in 2023 and his bachelor degree in software engineering from Wuhan University of Technology in 2020. He is currently working as an AI engineer at Huawei Technologies Co. Ltd. His research interest is on generative tasks such as face swapping and frame prediction. 
%\vspace{-1cm} 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_zy.jpeg}}]{Yong Zhang}
is currently a senior researcher in Tencent AI Lab. His research is on AIGC (AI Generated Content), e.g., image and video generation. Before joining Tencent, he received  Ph.D. degree from Institute of Automation, Chinese Academy of Sciences (CASIA) in 2018 and was supervised by Prof. Bao-Gang Hu and Prof. Weiming Dong at National Laboratory of Pattern Recognition (NLPR). Prior to CASIA, he got B.Eng in Automation from Hunan University in 2012. From Sep. 2015 to Sep. 2017, he was a joint Ph.D. student in the Intelligent System Lab (ISL) at Rensselaer Ploytechnic Institute (RPI).
\vspace{-1cm} 
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_nyw.jpg}}]{Yongwei Nie}
is now an Associate Professor at the School of Computer Science and Engineering of South China University of Technology, Guangzhou, Guangdong, China, 510006. He received his doctor and bachelor degree from Computer School of Wuhan Univesrity in 2015 and in 2009. His research interests fall in Computer Graphics and Computer Vision.
\vspace{-1mm} 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_wj.jpeg}}]{Jue Wang}
Jue Wang (Fellow, IEEE) received the BE and MSc degrees from the Department of Automation, Tsinghua University, Beijing, China, in 2000 and 2003, respectively, and the PhD degree in electrical engineering from the University of Washington, Seattle, Washington, in 2007. He has published more than 200 research articles in top-tier academic journals and conferences in the areas of Computer Vision, Computer Graphics, Machine Learning and HCI, and holds more than 80 international patents. He is Associated Editor for IEEE Transactions on Pattern Analysis and Machine Intelligence (T-PAMI).
He is currently co-founder on a startup, Beijing, China. 
Prior to this new adventure, he was Distinguished Scientist at Tencent, leading research efforts in intelligent content generation for the gaming and entertainment industry. He was the Director of the Visual Computing Center at Tencent AI lab, a multidisciplinary research hub for Computer Vision, Computer Graphics and HCI. He was Senior Director at MEGVII Research from 2017 to 2020, and was Principal Scientist at Adobe Research from 2007 to 2017.
\vspace{-1mm} 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/bio/bio_xd.jpeg}}]{Dong Xu} (Fellow, IEEE) 
received the B.Eng. and PhD degrees from University of Science and Technology of China (USTC), in 2001 and 2005, respectively. While pursuing the PhD degree, he worked at Microsoft Research Asia as an intern and The Chinese University of Hong Kong as a research assistant for more than two years. He also worked as a postdoctoral research scientist at Columbia University, a tenure-track and tenured faculty member at Nanyang Technological University, and Chair in Computer Engineering at The University of Sydney.
His current research interests include computer vision, multimedia, and machine learning. His group has developed new machine learning methods and intelligent systems for a broad range of vision and multimedia related applications such as autonomous driving, AR/VR, video compression and surveillance, as well as medical image analysis. He has published more than 150 papers in IEEE Transactions and leading conferences including CVPR, ICCV, ECCV, ICML, ACM MM and MICCAI. His co-authored works (with his former PhD students) received the Best Student Paper Award in CVPR 2010 and the IEEE Transactions on Multimedia Prize Paper Award in 2014.

\end{IEEEbiography}




\clearpage
